Spreading of highly cohesive metal powders with transverse oscillation kinematics

Powder bed additive manufacturing processes such as laser powder bed fusion (LPBF) or binder jetting (BJ) benefit from using fine (D50 $\leq20~\mu m$) powders. However, the increasing level of cohesion with decreasing particle size makes spreading a uniform and continuous layer challenging. As a result, LPBF typically employs a coarser size distribution, and rotating roller mechanisms are used in BJ machines, that can create wave-like surface profiles due to roller run-out. In this work, a transverse oscillation kinematic for powder spreading is proposed, explored computationally, and validated experimentally. Simulations are performed using an integrated discrete element-finite element (DEM-FEM) framework and predict that transverse oscillation of a non-rotating roller facilitates the spreading of dense powder layers (beyond 50% packing fraction) with a high level of robustness to kinematic parameters. The experimental study utilizes a custom-built mechanized powder spreading testbed and X-ray transmission imaging for the analysis of spread powder layers. Experimental results generally validate the computational results, however, also exhibit parasitic layer cracking. For transverse oscillation frequencies above 200 Hz, powder layers of high packing fraction (between 50-60%) were formed, and for increased layer thicknesses, highly uniform and continuous layers were deposited. Statistical analysis of the experimental powder layer morphology as a function of kinematic spreading parameters revealed that an increasing transverse surface velocity improves layer uniformity and reduces cracking defects. This suggests that with minor improvements to the machine design, the proposed transverse oscillation kinematic has the potential to result in thin and consistently uniform powder layers of highly cohesive powder.

==> old_chapters/conclusion.tex <==
\section{Conclusion}

% % Work in this paper
% This work investigates the spreading of very cohesive powder in PBF using a roller implement through computational simulations.
% Compared to spreading with a blade, using a counter-rotating roller allows to create thin powder layers of high quality with fine, cohesive powders when optimizing the kinematic parameters. This indicates that there is a material-specific process window for the deposition of these cohesive powders.
% For the investigated representative 0-20~$\mu m$ Ti-6Al-4V powder, high counter-rotating angular velocities of 500 rpm, a friction coefficient of the roller of over 0.4 and moderate traverse velocities of around 10-25~$\frac{mm}{s}$ achieved best results. The high level of shear and the moderate deposition rate allow for a uniform and dense layer.
% As experimentally shown by Penny et al.~\cite{PENNY2022Roller}, a high manufacturing precision for the spreading apparatus is required in order to avoid a wave-like surface profile coming from the runout of the rotating roller. To mitigate the difficulty of manufacturing with such high precision, oscillation spreading patterns in angular direction and perpendicular to the spreading direction are proposed. Employing a frequency of approx.~500 Hz and an amplitude of 1$^{\circ}$ (corresponding to a value just larger than the largest particle diameter) showed best results, with a powder bed density that was higher than what was achieved with an angular rotation (52.2\% vs. 48.1\%). Furthermore, using very high frequencies (10 kHz or larger) in combination with very small amplitudes (i.e., 0.1$^{\circ}$) was shown to be less effective.
% When analyzing the impact of different properties of the underlying layer by means of a reduced level of adhesion of the substrate, it was shown that the spreading conditions that produce best results on a substrate that has similar cohesive properties as the powder also produce best results on a less cohesive substrate. For example, when reducing the substrate adhesion by a factor of 10, the powder bed density stays consistent when using the best parameter set for a default surface adhesion.
% On the other hand, one could also imagine using different materials for the roller. For the limiting case of no adhesion of the powder to the roller, no significant impact was seen on the powder layer quality, when employing the best spreading parameter set as derived for a roller with a normal level of adhesion.
% As another option to improve the spreading tool, flexible blades are known to mitigate singular defects such as streaking. While these singular effects are commonly not observed in computational work, we assume that it can be generalized from computational results. The examination of a rubber-coated roller showed no negative impact on powder layer quality. This is a positive result, as it shows that even the dynamic spreading patterns of angular oscillation are stable using compliant tools, while offering the benefit of mitigating singular effects such as streaking.
% Changing the geometry of the spreading tool to a larger roller decreased the powder layer quality, indicating that the optimal parameters for one geometry don't necessarily translate directly to a similar spreading geometry of different scale.
% Lastly, we analyzed oscillating the roller not in angular direction, but perpendicular to the spreading direction. This approach yielded comparable results to the angular oscillation and offers a viable alternative to the other proposed spreading approaches in this work.

% In conclusion, the proposed angular or traverse oscillation patterns with a compliant spreading tool and a high ratio of oscillation to traverse velocity are a very promising avenue with the following key benefits:
% \begin{itemize}
%     \item high and uniform packing density in the range between 50 and 60 percent
%     \item robust w.r.t. varying substrate conditions (e.g., reduced substrate adhesion)
%     \item no runout problems as compared to pure rotation kinematics
%     \item oscillation can even be extended to non-roller geometries
%     \item compliant coating mitigates problems due to collisions or streaks
%     \item powder layer quality further improves with increasing nominal layer thickness
% \end{itemize}

% % Future Work
% For future work we see primarily two directions. First, the computationally examined concepts in this work need to be experimentally verified in order to be used by practitioners. Second, the less common hopper-based powder deposition approach should be analyzed in depth as well. Since it usually requires a smoothing pass with a tool, it might also benefit from the concepts described in this work.

Using a coupled DEM-FEM computational model, this work investigates the spreading of very cohesive powders, as required e.g. in LPBF or BJ additive manufacturing, by means of a roller implement. Compared to spreading with a blade, using a counter-rotating roller allows to create thin powder layers of high quality with fine, cohesive powders when optimizing the kinematic parameters. This indicates that there is a material-specific process window for the deposition of these cohesive powders. For the investigated highly cohesive 0-20~$\mu m$ Ti-6Al-4V powder, high counter-rotating angular velocities of 500~rpm, a large enough friction coefficient of the roller surface of $\mu \geq 0.4$ and moderate traverse velocities of around 10-25~$\frac{mm}{s}$ achieved best results. For angular velocities $<$500~rpm (and also for too low values of the roller friction coefficient $\mu$) insufficient kinetic energy is induced into the powder as to effectively break cohesive bonds, while for  angular velocities $>$500~rpm the induced kinetic energy is too high, leading to significant particle ejection and a pronounced "dusty zone" in front of the roller, both resulting in reduced packing fraction values as compared to the optimal case with $\omega = 500$~rpm. As experimentally shown by Penny et al.~\cite{PENNY2022Roller}, a high manufacturing precision for the spreading apparatus is required in order to avoid a wave-like surface profile coming from the runout of the rotating roller. To mitigate the difficulty of manufacturing with such high precision, oscillation spreading patterns in angular direction and transverse to the spreading direction are proposed. Here, oscillation amplitudes in the order of the diameter of the largest particles in the powder size distribution (corresponding to an amplitude of approximately 1$^{\circ}$ when considering angular oscillations with the given roller dimensions and powder size) showed best results. Interestingly, both angular and transverse oscillations yielded the best layer quality when the oscillation frequency was chosen such that the resulting maximal (circumferential or transverse) velocity on the roller surface is comparable to the counter-rotating case with optimal angular velocity $\omega = 500$~rpm. Critically, all these spreading approaches, i.e., counter-rotation as well as angular and transverse oscillation, are shown to be very robust with respect to varying substrate conditions (e.g., reduced substrate adhesion by one order of magnitude), which are likely to occur in LBPF or BJ, where substrate characteristics are the result of a complex multi-physics (i.e., powder melting or binder infiltration) process. Specifically, angular and transverse oscillation kinematics showed a high level of robustness regarding kinematic parameters (i.e., high layer quality across a wide range of frequencies) as well as substrate conditions.
While the present study considered the most challenging case of rather thin layers (layer thickness of approx. D90) of highly cohesive powers, it was demonstrated that higher packing fraction levels can be achieved for thicker layers, an effect that is well-known from previous studies. On the other hand, parameters such as the roller diameter (for a fixed value of the maximal circumferential velocity on the roller surface) and the powder-to-roller adhesion (controllable, e.g., through the roughness and material of the roller surface) were shown to have less influence on the layer quality as compared to the roller kinematics, at least in the regime of optimal angular / oscillation velocities. 

In conclusion, the proposed angular and transverse oscillation patterns on roller-like geometries with oscillation amplitudes in the order of the largest particles in the powder size distribution, a sufficiently rough surface of the spreading tool (coefficient of friction above 0.4) and a low to moderate traverse velocity are recommended. Optimal oscillation frequencies have to be determined based on the cohesiveness of the given powder material such that the induced kinetic energy is high enough to break adhesive bonds but not too high, which would result in excessive particle ejection. In sum, the following key benefits can be stated:
\begin{itemize}
    \item high and uniform packing densities beyond 50 percent even for very thin layers of highly cohesive powders
    \item robustness w.r.t. varying substrate conditions (e.g., reduced substrate adhesion)
    \item robustness w.r.t. deviations from the optimal oscillation frequency (more robust than pure counter-rotation)
    \item no runout problems as compared to pure rotation kinematics
    \item oscillation can be extended to non-roller geometries
\end{itemize}

Apart from different roller kinematics, also first studies on the usage of composite recoating tools, e.g. rubber-coated rollers, have been performed. Fully compliant recoating tools (e.g. made of rubber) are well-known to reduce the risk of tool damage and quality-degrading singular effects such as streaking of large particles, but typically the achievable manufacturing tolerances are not sufficient to allow, e.g., for counter-rotation roller spreading. A promising alternative has been proposed in this work by applying oscillatory kinematics (which are less restrictive w.r.t. manufacturing tolerances) to a rubber-coated steel roller combining the advantages of stiff and compliant spreading tools (i.e., kinematic precision and robustness). Our preliminary studies confirmed that such rubber-coated rollers allow to precisely control oscillatory surface kinematics and to achieve a comparable packing density and layer uniformity as with steel rollers as long as no singular effects such as particle streaking occur (which rarely happens on the domain sizes typically considered in computational modelling). Therefore, the usage of such rubber-coated rollers, and in particular the analysis of their robustness w.r.t. collisions and streaking, are considered as very promising avenues of future research. In addition, our future research will also focus on an experimental validation of the proposed spreading approaches.



==> old_chapters/introduction.tex <==
\section{Introduction}

The powder deposition process is a critical step for powder-bed based metal additive manufacturing (AM) processes, such as binder jetting (BJ) and laser powder bed fusion (LPBF), because the powder layer directly impacts the resulting part quality~\cite{MIAO2022103029}, production rate~\cite{li2020metal}, and geometrical resolution/feature size~\cite{fang2023state}.

For both processes, the typical setup includes a powder reservoir (usually driven by a piston or a movable hopper), a powder bed, and a spreading tool such as a blade or roller.
The initial step in LPBF processing involves raising the powder reservoir to provide a predetermined volume of powder. Concurrently, the build platform is lowered to receive a new layer of powder with a thickness corresponding to the nominal layer thickness. Following this, the spreading tool distributes the powder from the reservoir onto the build platform, forming a new powder layer over the previous layer, or for the first layer over the substrate. Once the powder spreading operation is complete, a laser selectively fuses particles within the powder bed to consolidate the desired geometry~\cite{meier2017thermophysical, MIAO2022103029, wang2024review}. In the case of binder jetting (BJ), a liquid binder is applied on the fresh powder layer to establish connections between adjacent particles, resulting in the formation of the 'green part,' which is then sintered to produce the final component~\cite{fang2023state, li2020metal}.


% From Thesis:

% Powder bed metal additive manufacturing (AM) technologies are making it possible to create intricate, high-performance components for various applications, including aerospace propulsion systems and medical implants~\cite{SpaceX2024, James2021, dias2024unveiling}. These powder bed AM techniques construct parts incrementally, layer-by-layer, by bonding or melting successive cross-sections. Thus, the initial step in the recurrent cycle of building a part is the powder deposition process, and the quality of the powder layer significantly influences both the quality of the part and the overall efficiency of the process.

% Two of the most widespread metal additive manufacturing technologies are laser powder bed fusion (LPBF) and binder jetting (BJ). Both techniques typically involve a powder reservoir, a build platform, and one or more tools for distributing the powder. In a standard LPBF setup, the powder reservoir platform is elevated by a piston to deliver a specified amount of powder initially, while the build platform lowers by the designated nominal layer thickness to gather fresh powder. The spreading tool then moves the powder from the reservoir onto the build platform, establishing a new layer atop the previous one or the substrate. Once the powder is spread, a laser selectively melts particles in the powder bed~\cite{capozzi2022powder}. 
% In BJ setups, a hopper usually replaces the piston-driven reservoir. The hopper administers the initial powder supply over the build platform or continuously in front of the spreading tool, which subsequently forms a layer on the platform. Then, a liquid binder is deposited via inkjet printing, connecting adjacent particles in specific areas to form the 'green part', which is later extracted from the printer and sintered to produce the finished part~\cite{li2020metal}.

% In both processes, the powder layer influences (i) the final part's quality, since imperfections in the powder can manifest in the finished product~\cite{MIAO2022103029}, (ii) production speed, which is affected by the layer's thickness and the speed at which it is spread~\cite{li2020metal}, and (iii) the attainable geometric resolution, limited by the particle size and layer thickness.

\subsection{Fine Powders in AM} 

The feedstock material in powder-based AM is usually driven by both the application as well as the ability to process a certain material. Since the dominant use cases of metal AM so far have been in aerospace and healthcare, the most widely used materials are nickel-based superalloys such as In625, titanium alloys such as Ti-6Al-4V, steel such as SS316, and aluminum alloys such as Al-Si10-Mg~\cite{qian2015metal, li2020metal, avrampos2022review}. Additionally, new materials are being developed specifically for processing in metal AM, including multi-material processing strategies~\cite{li2019progress, demir2022enabling}.
Because they show beneficial processing properties, spherical particles have become the standard in metal AM -- usually manufactured by plasma atomization or gas atomization~\cite{Boley2016MetalExperiment, Tan2017AnProcess, Mukherjee2016, Gu2012}.

Most commercial LPBF machines, as well as most research in LPBF utilizes or focuses on powders in the range from 15-60~$\mu m$, or even coarser, and existing literature consistently reports challenges with spreading finer, more cohesive powders~\cite{Wu2023, MIAO2022103029,li2020metal, Vock2019}. BJ processing requires finer powders for better sintering characteristics as well as binder absorption and thus usually has to resort to agitated hopper designs in combination with a roller~\cite{li2020metal, bai2015effect, Ziaee2019, Lores2019}, but also LBPF would benefit from using finer powders to improve geometric resolution. 

The main reasons that render a powder difficult to handle are non-spherical morphology of the particles, humidity, and adhesive surface forces. For finer particles, adhesive forces become larger than inertia forces, which leads to challenges in spreading thin powder layers~\cite{Walton2007, Walton2008, Herbold2015, Kloetzer2004ProcessCVD, Meier2019CriticalManufacturing, weissbach2024exploration}. Recycling powder further increases challenges with powder handling, and thus often requires sieving the powder before adding it back to the processing cycle~\cite{Cordova2019, avrampos2022review}. 



% Summarize the below sections to shorten

\subsection{Spreading instruments and kinematics}

Machines for powder bed-based metal AM typically spread powder using a blade (most common for LPBF) and/or a roller (most common for BJ)~\cite{Haeri2017,Haeri2017_2,Snow2019}, to create layers with a typical thickness of $\sim$30-120$~\mu m$~\cite{Gibson2010, Vock2019}. The quality of the layer (e.g., uniformity, density, surface roughness), is primarily dependent on the feedstock properties and the geometry and kinematic motion of the spreading tool. 
%Layer thickness
Previous work has shown that the packing fraction of the powder bed increases with increasing layer thickness~\cite{yao2021dynamic,nan2020a, Meier2019CriticalManufacturing, zhang2020, Mindt2016}, and reaches saturation at a value that is around 55-60\%.
More specifically, it has been shown that the nominal layer thickness should exceed $1.5\times D_{90}$, where $D_{90}$ is the 90\textsuperscript{th} percentile of particle diameters to avoid streaking of the layer, which is caused by the largest particles in the distribution~\cite{Spierings2011}. Accordingly, this work will employ a layer thickness of over $1.5\times D_{90}$. As a reference for typical packing fractions in high quality processes, an exemplary study reported 53\% average packing fraction for 28-48~$\mu m$ Ti-6Al-4V powder in a LPBF machine~\cite{Wischeropp2019}, which is sufficient for stable LPBF processing~\cite{Ziaee2019}.

%Traverse velocity
Rapid spreading is desirable to increase throughput, but the blade or roller velocity has been shown to have significant impact on the resulting layer quality. According to several studies, the packing fraction first is low for slow traverse velocities ($<$10$\frac{mm}{s}$), peaks, and then decreases significantly for high spreading velocities~\cite{Chen2017, Snow2019, yao2021dynamic, Haeri2017, chen2020packing, zhang2020}. Additionally, the surface uniformity of powder layers consistently decreases with increasing traverse velocity~\cite{Meier2019CriticalManufacturing, Parteli2016, Haeri2017, PENNY2022Blade, PENNY2022Roller}. For example, increasing the traverse velocity from 127$\frac{mm}{s}$ to 607$\frac{mm}{s}$ with a blade tool significantly decreased the packing fraction and surface uniformity of relatively coarse (PSD of 0-125~$\mu m$) polymer powders~\cite{Meyer2017}.
Potential sources for this behavior are bridging effects (i.e., particles build a stable force chain that 'bridges' the gap) and particle inertia both during feeding through the spreading gap as well as post-spreading inertia~\cite{chen2020packing, Meier2019CriticalManufacturing, Wang2021}.

%Tool
As mentioned above, common spreading implements used in powder bed AM are blades and rollers. For blades, which are typical in LPBF due to the larger and less cohesive powders used, round edges achieve higher packing fractions and higher uniformity than blades with a sharp edge~\cite{Meyer2017, Wang2021, Haeri2017}. Using a roller for spreading, with transverse motion and counter-rotation, typically leads to a higher packing fraction than a blade under otherwise identical powder and spreading conditions, as shown by~\cite{Haeri2017, wang2020, shaheen2021influence, zhang2020, Budding2013, PENNY2022Roller}, which can be explained by a circulation of particles in the pile in front of the spreading tool, allowing a better rearrangement before being deposited~\cite{nan2020a}. Further factors such as roller diameter and roughness of the surface also influence the quality of the powder bed, as shown by Oropeza et al.~\cite{oropeza2022mechanized} who used X-ray microscopy to image the spatial distribution of packing density within layer spread with a mechanized apparatus. Forward-rotating roller kinematics have also been proposed as a means to densify the powder layer. However, there are considerable drawbacks associated with forward-rotation, primarily the significantly higher and strongly varying forces exerted on the powder bed. In LPBF, high local forces exerted by the spreading tool can damage thin and delicate printed features. In BJ, the structural integrity of the green part is low, leading to a risk of shear deformation~\cite{niino2009effect} or deteriorating the weakly bound powder structure (leading to e.g., cracking)~\cite{li2021binder}. The powder bed can also be elastically deformed as a co-rotating roller passes, leading to a subsequent release of said elastic energy in the form of springback. This can lead to a thicker layer than intended and non-uniform surface profiles~\cite{ziaee2019fabrication}. A combination of counter-rotation and angular oscillation was first explored by Seluga~\cite{seluga2001} and showed promising results of improved packing fractions compared to pure counter-rotation when parameters are chosen correctly.
In \cite{nasato2021influence}, vertical oscillation is applied to DEM simulations of blade and roller spreading of a PA~12 powder. It was shown that for most scenarios, vertical oscillation of the spreading tool reduces powder layer quality.

The spreading tool can also become worn and damaged over repeated use, especially as consequence of non-uniform forces due to warpage of the part especially in LPBF, and interaction with agglomerates or solidified spatter. This damage, in turn, leads to tool vibrations resulting in layer defects~\cite{Vock2019, Hendriks2019}. Among others, this motivates the frequently used choice of compliant spreading tools, which accommodate high local forces with elastic deformation of the tool edge/surface. 
% Taken together, the dynamics of the spreading tool and uncertainties in powder properties (e.g., due to input variation, and implications of powder reuse) lead to a significant variance in the layer properties, namely the packing fraction. 

\subsection{Powder spreading simulations --> work into previous section}

Given the complex dynamics of powder spreading and the challenge of directly observing powder flow at the submillimeter length scales involved in spreading, computational modeling can lead to new insights that guide the development of practical methods and spreading mechanisms for improvement of AM processes. 
Pioneering works~\cite{Mindt2016, Herbold2015, Haeri2017, Gunasegaram2017} showed the suitability of discrete element method (DEM)~\cite{Luding2006,Luding2008} simulations to study the powder spreading process in LPBF. The authors showed in \cite{Meier2019CriticalManufacturing} the importance of considering cohesion for powder spreading, and a calibration strategy for the cohesive surface energy via angle of repose (AOR) experiments was presented in~\cite{Meier2019ModelingSimulations}. Referring to~\cite{Meier2019ModelingSimulations, Meier2019CriticalManufacturing}, several subsequent works adopted the approach to modeling and calibration of cohesion~\cite{Lee2020,HAN2019,wang2020,nan2020a,he2020,KOVALEV2020,zhang2020}. These previous contributions simulated spreading of polydisperse, spherical or non-spherical powders, considered visco-elastic contact, friction, rolling resistance, cohesion and fluidization~\cite{nan2020b} as particle interactions, and predicted layer properties such as packing fraction, surface uniformity and particle segregation in dependence of layer thickness, spreading velocity and spreading tool geometry~\cite{desai2019,shaheen2021influence}. It was shown that critical parameters are tool geometry, layer thickness, spreading kinematics, particle shape, and most importantly the level of cohesion, as described above. Despite various numerical studies that have focused on the powder spreading process so far, there is still a gap regarding strategies that enable the spreading of highly cohesive powders. 


\subsection{Overview}

This paper presents an in-silico study of the complex multi-physics problem of spreading highly cohesive powders with a roller by utilizing an integrated DEM-FEM framework. 
In particular, the computational studies explore roller kinematics including counter-rotation as well as angular and transverse oscillation applied to standard rigid rollers as well as coated rollers with compliant or non-adhesive surfaces. 
We find that optimal roller-based spreading, quantified by the packing density and uniformity of layer thickness, relies on a combination of surface friction of the roller and roller kinematics that impart sufficient kinetic energy to break cohesive bonds between powder particles. However, excess rotation (or shear stress) can impart excessive kinetic energy to the powder causing ejection of particles and a non-uniform layer.
When these conditions are chosen appropriately, high packing fractions beyond 50~\% are predicted for layer thicknesses as small as $\sim$2 times D90 of the exemplary powder, and the layer quality is robust with respect to substrate adhesion over a 10-fold range which is an important consideration given the spatially varying substrate conditions in AM due to the combination of fused/bound and bare powder regions. Moreover, parametric DEM-FEM simulations allow us to identify new spreading strategies combining rollers with surfaces with reduced adhesion and/or compliant surface coatings, and angular and/or transverse oscillation during spreading. Roller oscillation is particularly attractive because it can overcome practical issues with mechanical runout of roller mechanisms (which limit their precision), and is recommended for future experimental investigation.

The structure of this work is as follows. Section~\ref{sec:Methods} gives background the central elements of the DEM-FEM model and describes the simulation setup, the quality metric as well as the employed model parameters. Subsequently, Section~\ref{sec:Results} reports the results of computational studies. Based on an initial comparison of blade vs. roller spreading for different levels of powder cohesion, one selected level of cohesiveness is investigated in the remainder of the study. We assess the influence of traverse and rotational velocity as well as the roller friction coefficient in pure counter-rotational roller spreading. The results are then compared to an analysis of frequency and amplitude in spreading with angular oscillation as well as traverse oscillation, including spreading over a substrate with a reduced surface energy (by factor of 10 lower). The angular rotational and oscillation cases are extended to scenarios with a coated roller where particles do not adhere to, spreading with a flexible rubber-coated roller, spreading layers where the layer thickness is doubled, and spreading with a roller where the diameter is doubled. Finally, the results are discussed and put into perspective in the conclusion.

 



==> old_chapters/methods.tex <==
\section{Computational Methods}
\label{sec:Methods}

The computational methods used in this work are the same as those applied in our previous publication focused on computational roller spreading~\cite{weissbach2024exploration}. As recommended by \cite{Nature2024} the following description of computational methods is largely reused from \cite{weissbach2024exploration}.

\subsection{Computational Model}

Spreading of fine metal powders is simulated via an integrated discrete element method-finite element method (DEM-FEM) framework that was first described in \cite{Meier2019ModelingSimulations}, implemented in the parallel multi-physics research code BACI~\cite{Baci}. This model has also been applied in~\cite{Meier2019CriticalManufacturing, Meier2021GAMM, Penny2021,PENNY2022Blade,PENNY2022Roller}, but this is the first in-depth study of roller spreading for fine powders. Each particle is modeled as a discrete spherical element. Structural elements, such as the spreading tool or the substrate are modeled via FEM elements. Bulk powder dynamics are described with the resolution of individual particles following a Lagrangian approach. The model considers particle-to-particle and particle-to-wall (e.g., tool and substrate) interactions including normal contact, frictional contact, rolling resistance and cohesive forces.

Each discrete element (i.e., particle) has six degrees of freedom (i.e., three translational and three rotational DOFs) described by the position vector $\mb{r}_G$ and the rotation vector $\boldsymbol{\psi}$ and angular velocity $\boldsymbol{\omega}$ of the centerpoint of a particle. Based on these, the balance of momentum equations of a particle $i$ are~\cite{Meier2019ModelingSimulations}:
\begin{subequations}
\label{momentum}
\begin{align}
(m \, \ddot{\mb{r}}_G)^i = m^i \mb{g} + \sum_j (\mb{f}_{CN}^{ij}+\mb{f}_{CT}^{ij}+\mb{f}_{AN}^{ij}),\label{gusarov2007_HCE1}\\
(I_G \, \dot{\boldsymbol{\omega}})^i = \sum_j (\mb{m}_{R}^{ij}+\mb{r}_{CG}^{ij} \times \mb{f}_{CT}^{ij}),\label{gusarov2007_HCE2}
\end{align}
\end{subequations}
with the particle mass $m\!=\!4/3\pi r^3\rho$, the moment of inertia with respect to the particle centerpoint $I_G=0.4mr^2$, the particle radius $r$, the density $\rho$, and the gravitational acceleration $\mb{g}$. A bold symbol indicates a vector and a dot above a parameter indicates the derivative with respect to time of said parameter, e.g., $\dot{\boldsymbol{\omega}}^i$ is the angular acceleration vector of a particle $i$.
Each contact interaction between particles $i$ and $j$ is represented in Eq.~\eqref{momentum} through normal contact forces $\mb{f}_{CN}^{ij}$ (implemented with a spring-dashpot model), tangential contact forces due to Coulomb's friction $\mb{f}_{CT}^{ij}$ (with stick/slip frictional contact), adhesive forces $\mb{f}_{AN}^{ij}$, and torques $\mb{m}_{R}^{ij}$ due to rolling resistance. Furthermore, $\mb{r}_{CG}^{ij}:=\mb{r}_{C}^{ij}-\mb{r}_{G}^i$ is the vector pointing from the centerpoint of particle $i$ to the contact point with particle $j$. 

Our previous work~\cite{Meier2019ModelingSimulations, Meier2019CriticalManufacturing} showed that cohesive forces between particles dominate the dynamics and spreadability of micron-scale metal powders. 
In~\cite{Meier2019ModelingSimulations}, a cohesion force law according to the Derjaguin-Muller-Toporov (DMT) model~\cite{Derjaguin1975}, was proposed and the interested reader is referred to that reference for more details on the formulation. The surface energy $\gamma$ has is a critical parameter due to (i) high uncertainty about the magnitude and variance between particles (by several orders of magnitude due to variations in particle surface roughness/topology and chemistry); and (ii) high influence on the powder behavior such as flowability and spreadability. For example, for effective surface energy values on the order of $\gamma=1$e-4$~\frac{J}{m^2}$ as identified for representative powders~\cite{Meier2019CriticalManufacturing} and mean particle diameters in the range of $d=2r \approx 30~\mu m$, cohesive forces are 10-fold greater than gravitational forces.


\subsection{Simulation setup}
\label{subsec:simulation setup}

The following geometric setup is used for the simulation of powder spreading with a roller, with powder supplied by a reservoir as described below. The roller is modeled based on 125 linear circumferential segments of a circle with a diameter of 10~mm. For roller simulations, 42,000 particles are used. This number was chosen based on a sensitivity study and represent the threshold where a larger number did not significantly affect simulation results.
The dimensions of the powder reservoir and powder bed are similar to those used in previous work~\cite{Meier2019ModelingSimulations,Meier2019CriticalManufacturing, Meier2021GAMM, Penny2021,PENNY2022Blade,PENNY2022Roller}: the dimension perpendicular to the spreading direction is 1~mm with periodic boundary conditions, the powder bed has a length of 12~mm and quality metrics are evaluated over a 5~mm length, starting 3~mm after the beginning of the powder bed to avoid potential edge effects in the beginning or the end. The thickness of the layer is defined by the gap between the bottom edge of the spreading tool and the substrate, and is set to be $\sim$2 times the D90 particle diameter and just slightly thicker than the largest particle in the distribution (e.g., 100~$\mu m$ for a 15-45~$\mu m$ powder with a cutoff diameter of 88~$\mu m$ or $\sim$40~$\mu m$ for a 0-20~$\mu m$ powder as described below). In the beginning of the simulation, particles are randomly allocated on a grid in the powder reservoir. The particles drop down due to the gravitational force and the powder reservoir piston moves the pile of powder up and in front of the spreading tool. This situation is depicted in Figure~\ref{fig:simulation_setup}, just before the spreading tool starts to move across the powder bed.

\begin{figure}
\vspace{-12pt}
 \begin{center}
   \includegraphics[scale=1, keepaspectratio=true, width=\textwidth]{Figs/simulation_setup_v2.png}
 \end{center}
 \vspace{-16pt}
 \caption{Simulation setup with roller, fully extended powder reservoir piston with 42,000 particles and powder reservoir}
   \vspace{-12pt}
 \label{fig:simulation_setup}
\end{figure}


\subsection{Quality metric: Spatially resolved packing fraction}

The primary layer quality metric analyzed in this work is the 2D packing fraction field $\Phi$ of the powder bed, quantified by its mean $\bar{\Phi}$ and standard deviation $std(\Phi)$. The computation and motivation of this metric is described in detail in \cite{Meier2019CriticalManufacturing} and will only be covered briefly here. This metric is assessed with a spatial resolution of 100x100~$\mu m$ in the length and width direction (denoted as bins), which is approximately the diameter of a typical laser spot in LPBF. For example, a low standard deviation of the packing fraction field indicates a high level of uniformity. The packing fraction is evaluated in two steps. First, each bin is further divided into smaller cubical 3D voxels with a side length of 2.5~$\mu m$ for a numerical integration of the particle volume. The voxel size is chosen as to minimize the error coming from the volume of particles cut by the segment walls. Finally, the packing fraction of the powder layer is evaluated as the ratio of the volume occupied by particles to the volume of the powder bed confined by the actual mean layer height. 

\textit{Remark:} For the calculation of the packing fraction, the nominal layer height is commonly employed in the literature. We do not use the nominal layer height but the actual (calculated) mean layer height. This is important since the nominal layer height usually is considerably higher than the actual mean layer height of a spread layer. The mean layer height is calculated as the mean value of the layer heights of all 100~$\mu m$ bins~\cite{Meier2019CriticalManufacturing}.

\subsection{Powder model parameters}
\label{subsec:Powder model parameters}

The particle size distribution (PSD) was fitted to experimental laser diffraction measurements in our previous work~\cite{Penny2021}, and the same values for the $10^{th}$-percentile (D10), median (D50) and $90^{th}$-percentile (D90) are fitted to a lognormal distribution in this work (D10~=~23.4~$\mu m$, D50~=~31.5~$\mu m$, D90~=~43.4~$\mu m$; cutoff diameter D$_{cutoff}$~=~88~$\mu m$). Most other powder model parameters are also kept the same as referenced in~\cite{Penny2021,PENNY2022Blade,PENNY2022Roller}, and are listed in Table~\ref{tab:DEMparameters}.

This work focuses on evaluating powders with a high level of cohesion. Cohesive forces in the model are primarily determined by the surface energy $\gamma$ of the particles. A higher value of $\gamma$ defines a more cohesive powder. In \cite{Meier2019ModelingSimulations}, we showed that the critical dimensionless group that defines the cohesiveness of a powder is the ratio of gravitational and adhesive forces, which scales according to:
\begin{align}
    \frac{F_{\gamma}}{F_g} \sim \frac{\gamma}{\rho g r^2}.% \overset{!}{=} const.
\label{eq:Gravitation to Cohesion}
\end{align}
As shown in \cite{Meier2019ModelingSimulations}, the behavior of a given powder is similar as long as the ratio stays constant. For example, a powder with a lower density, such as an aluminum alloy, and a larger size distribution might behave similar to a higher density metal, such as steel, with a smaller size distribution.
Making use of this self-similarity condition, one can model the behavior of a powder based on the known behavior of others. The present model was calibrated on the 15-45~$\mu m$ Ti-6Al-4V powder (D10~=~20.2~$\mu m$, D50~=~27.0~$\mu m$, D90~=~36.0~$\mu m$), with a surface energy value of $\gamma_0$~=~0.08~$\frac{mJ}{m^2}$~\cite{PENNY2022Roller,PENNY2022Blade}. 
In this work, we aim to model a very fine powder that has the same surface energy as the previously calibrated 15-45~$\mu m$ Ti-6Al-4V powder. 
An exemplary commercially available 0-20~$\mu m$ Ti-6Al-4V powder with D10 = 7~$\mu m$, D50 = 10~$\mu m$ and D90 = 13~$\mu m$ matches this requirement and can be modeled by retaining the size distribution of the 15-45~$\mu m$ powder, while using a modified surface energy in the model that is calculated with the transformation rule
\begin{align}
    \gamma_{fine} = \left(\frac{D50_{coarse}}{D50_{fine}}\right)^2 \times \gamma_{coarse}.
\label{eq:powder cohesion transformation}
\end{align}
Using this transformation rule, the modified surface energy takes on a value of $\gamma = 8~\gamma_0$ or 0.64~$\frac{mJ}{m^2}$, i.e., the surface energy is increased by a factor of 8 as compared to its consistent physical value.
The same surface energy used to describe particle-particle interactions is also applied to particle-boundary interactions. 

\begin{table}
\centering
\renewcommand{\arraystretch}{0.7}
\begin{tabular}{ l l l } 
 \hline
 Parameter & Value & Unit \\ 
 \hline
 Density       &4430      &kg/m$^3$     \\ 
 Poisson's ratio     &0.342         &- \\
 Penalty parameter     &0.34         &N/m \\
 Coefficient of friction     &0.8         &- \\
 Coefficient of rolling friction     &0.07         &- \\
 Coefficient of restitution     &0.4         &- \\
 Surface energy     &0.64-1.28         &mJ/m$^2$ \\
 Hamaker constant     &$40\cdot10^{-20}$         &J \\
 Cut-off radius adhesion & $0.01$ & - \\
  \hline
 \end{tabular}
\caption{Default DEM model parameters}
\label{tab:DEMparameters}
\end{table}

Further, even though relatively cohesive metal powders have a significantly different flow behavior than coarse granular media such as dry sand, flow behavior of metal powders can be generalized more easily due to their relatively similar, high stiffness~\cite{Mandal2020}. Therefore, the findings of this study can be applied to other materials of significance to LPBF and BJ, as well as other processes requiring spreading of metal powders.

\subsection{Experimental Implementation}
\label{Experimental Implementation}

\begin{figure}
\vspace{-12pt}
 \begin{center}
   \includegraphics[scale=1, keepaspectratio=true, width=10cm]{Figs/Recoater VCM_iso.png}
 \end{center}
 \vspace{-16pt}
 \caption{Isometric view of the recoater equipped for transverse oscillation using a voice coil motor}
   \vspace{-12pt}
 \label{fig:Recoater iso}
\end{figure}

To allow for lower necessary forces to oscillate in the transverse direction, at the desired frequencies, notches were cut into the roller, thus reducing the mass from 200 g to 150 g. This reduced the necessary force to oscillate at the desired $\omega = 500 \, rpm$ equivalent velocity.

To stop the roller from rotating as it moves across the powder and build plates, a notch was cut into the end of the roller, allowing for a 3D printed rotational degree of freedom (DOF) stop that could be mounted to the top of the roller bearing housing.

For the spring constant combinations, there was a total of three different spring stiffnesses chosen, 57.792 [N/mm], 508.211 [N/mm], and 1911.166 [N/mm]. These were then put into five different combinations resulting in the following springs stiffnesses, resonant frequencies, and forces. Resonant frequency was calculated using  the following equation

\begin{align}
    \omega _n = \sqrt{\frac{k}{m}},
\label{eq:resonant freq}
\end{align}
where k and m are the spring constant and mass of the roller, respectively. Additionally, the force was calculated based on the following free body diagram and corresponding equation.

\begin{figure}
\vspace{-12pt}
 \begin{center}
   \includegraphics[scale=1, keepaspectratio=true, width=10cm]{Figs/voice coil FBD.PNG}
 \end{center}
 \vspace{-16pt}
 \caption{Free Body Diagram for roller during transverse oscillation}
   \vspace{-12pt}
 \label{fig:voicel coil FBD}
\end{figure}

\begin{align}
    F_{VC} = m \ddot x + b \dot x + k_T x,
    \label{eq: voice coil forces}
\end{align}
where m is mass, b is the damping experienced from friction (set to $1 \left[\, \frac{N \cdot s}{m}\right]$), and $k_T$ is the spring constant of both $S_1$ and $S_2$ combined. The motion of the controller is defined as 

\begin{align}
    x = A \, sin(\omega t),
    \label{eq: VC position}
\end{align}

here A is defined as the amplitude.

\begin{table}
\centering
\renewcommand{\arraystretch}{0.7}
\begin{tabular}{ l l l } 
\hline
 Spring combination $\left[\frac{N}{mm}\right]$ & Resonant frequency [Hz] & Force [N]\\ 
 \hline
 57.792       & 101.9091 & 0.1906 \\ 
 663.556     & 334 & 0.1588 \\
 1016.086     & 414.7273 & 0.2108 \\
 2419.202     & 636.7273 & 0.8408 \\
 3822.318     & 798.1818 & 2.3307 \\
\hline
\end{tabular}
\caption{Spring information}
\label{tab:springInfo}
\end{table}

\begin{figure}
\vspace{-12pt}
 \begin{center}
   \includegraphics[scale=1, keepaspectratio=true, width=10cm]{Figs/Force vs each spring const_50um.pdf}
 \end{center}
 \vspace{-16pt}
 \caption{Calculated force required to oscillate at varying frequencies and an amplitude of $50 \, \mu m$ for each combination of springs explored}
   \vspace{-12pt}
 \label{fig:force for springs}
\end{figure}
        
\textbf{Max frequency from the controller}
The controller has a maximum sample rate of 8kSa/s, allowing the voice coil motor (VCM) to be run reliably up to 1kHz. This is verified in the below figure.

\begin{figure}
\vspace{-12pt}
 \begin{center}
   \includegraphics[scale=1, keepaspectratio=true, width=7.5cm]{Figs/Sample vs true sine value_controller.pdf}
 \end{center}
 \vspace{-16pt}
 \caption{Comparing true VCM position value to the controller sample value}
   \vspace{-12pt}
 \label{fig:controller samples}
\end{figure}
        

The spreading abilities of the system were tested at \textbf{Insert tested velocities here}.
Layer thickness was verified with a depth gauge. The variation of thickness from one side of the roller to the other is less than $1 \, \mu m$.
The motor used is a Moticont SDLM-051-070-01-01 VCM which allows for a maximum continuous force of 30.3 N, a maximum intermittent force of 95.7 N, has a shaft stroke of 12.7 mm, and has an internal encoder with a resolution of 1.25 $\mu m$. The VCM is controlled by a Galil DMC-30012 motor controller. The motor controller does receive feedback from the VCM at a rate of 8kSa/s. Below is a high-level overview of the connections for the system:

\begin{figure}
\vspace{-12pt}
 \begin{center}
   \includegraphics[scale=1, keepaspectratio=true, width=7.5cm]{Figs/High level VCM Schematic.png}
 \end{center}
 \vspace{-16pt}
 \caption{Connection for operation between Galil GUI, motor controller and VCM}
   \vspace{-12pt}
 \label{fig:VCM and controller wiring}
\end{figure}

The roller straightness was measured with a Mitutoyo 293-705 digital micrometer, and was found to have a diameter of $\pm$ 57.15 $\mu m$.
The roughness of the roller was tested with a Keyence VK-X1000 3D microscope, and was found to have the following values.

\begin{table}
\centering
\renewcommand{\arraystretch}{0.7}
\begin{tabular}{ l l l l l l } 
\hline
 Sample Side & Ra $[\mu m]$ & Rz $[\mu m]$ & RSm $[\mu m]$ & R$\lambda$a $[\mu m]$\\ 
 \hline
 Side 1 (longitudinal)      & 2.525 & 24.830 & 1119.824 & 71.239 \\ 
 Side 1 (latitudinal) & 2.671 & 17.292 & 2535.546 & 173.285 \\
 Side 2 (longitudinal)    & 0.2.890 & 23.893 & 1244.447 & 79.541 \\
 Side 2 (latitudinal) & 2.776 & 17.440 & 1355.060 & 175.024 \\
\hline
\end{tabular}
\caption{(\textbf{Roughness of the powder roller, as measured by the Keyence VK-X1000 3D microscope}) or (\textbf{Ra being the average amplitude of all peaks and valleys, Rz being the maximum peak or valley value, RSm being the length measured of the sample, and R$\lambda$a being the average wavelength of the peaks and values})}
\label{tab:rollerRoughness}
\end{table}
The layer height variability was found using a depth gauge, and was tested at depths of 40 $\mu m$, 50 $\mu m$, 60 $\mu m$, 80 $\mu m$, and 100 $\mu m$. Comparing the distance measured between the roller and powder plate to the changes made in XI Lab (build/powder plate servo software), there was an $R^2$ value of 1 indicating good agreement between the closed-loop system and the method of verification. Comparing the distance measured between the roller and build plate to the changes made in XI Lab found and $R^2$ value of 0.986, again indicating good agreement between the two methods.
The lead screws operate on a closed-loop system with a motion controller (Synthetos tinyG). The velocity of the lead screws was verified with a Chronos 1.4 camera at 2000 fps, and was found to have $\pm \, 1 \%$ accuracy. The VCM also operates on a closed-loop system, with the aforementioned 8k sample rate. Verification with the Chronos 1.4 camera found an accuracy of

==> old_chapters/results.tex <==
\section{Results}
\label{sec:Results}

In what follows, we present parametric simulation studies focused on roller-based spreading of cohesive powders. We begin with comparing blade versus roller spreading for powders with different levels of cohesiveness as a benchmark comparison, then explore angular rotation, angular and transverse oscillation, as well as investigate the effect of reduced substrate adhesion and different modifications to the roller and simulation setup.
Each approach will be presented with motivation, parameter setup, and results. 
For the presented parameter studies, we found that halving the time step had no influence on the results, and therefore the timestep was kept the same in all presented simulations. Further, analysis of simulations using different seeds for the same parameters showed that the resulting statistical variation is significantly smaller than when comparing the results from the parameter study (see supplemental Figure~\ref{fig:seed_vs_original}).



\subsection{Roller-based spreading using angular oscillation}
\label{subsec:oscillation spreading}

Although spreading with a counter-rotating roller can be highly effective, practical outcomes are constrained by the manufacturing precision of the spreading apparatus~\cite{PENNY2022Roller}. Specifically, roller runout -- defined as non-circularity in the position of any reference point on the surface of the roller, as it rotates -- can impart a wavy profile in the powder layer, depending on the relative rotation and translation kinematics (see Figure 3 in~\cite{PENNY2022Roller}. Runout is caused by native imprecision in the roller geometry and its rotation, which is governed by the tolerances of machining, and those of mechanical components such as rolling element bearings as well as the overall assembly~\cite{oropeza2022mechanized}. As an approximation, for intended powder layers no greater than 100~$\mu m$ thickness, a roller manufacturing runout of only 10~$\mu m$ can significantly impact the local layer thickness and therefore the effective packing density. 
To potentially overcome this consideration, we used the simulation framework to study roller-based spreading with angular oscillations. By using only a segment of the roller surface, the effect of manufacturing runout is mitigated, as local variations over a small sector of the roller circumference are typically much less than the total circular runout.

Seluga in 2001 proposed for the first time an angular oscillation pattern~\cite{seluga2001}. In his work, a cohesive 0-15~$\mu m$ 17-4PH~SS powder is being coated with a polymer to make it less cohesive and spreadable. Subsequently, a custom-build spreading apparatus spreads powder with traverse velocities between 3-12$\frac{mm}{s}$ and an angular velocity of -60~rpm (i.e., counter-rotating). This motion is superimposed by a 60~Hz angular oscillation with varying amplitude. The superposition of the two rotational movements leads to two components of the relative velocity in the spreading gap. For small oscillation amplitudes, no effect on the packing fraction is observed. For higher amplitudes that lead to the relative velocity due to oscillation being larger than the relative velocity due to steady traverse and rotational movement, the packing fraction is significantly improved. The drawback is, that the surface of the powder layer is damaged with ridges due to a net-forward rotation of the roller during parts of the oscillation period. These ridges can be as deep as 30~$\mu m$ in a 50~$\mu m$ nominal powder layer, effectively rendering the layers unsuitable for LPBF or BJ processing. While the idea has not been utilized since due to the significant limitations in the study, the approach showed promising results.

Instead of a constant rotational velocity $\omega$, an oscillating rotational velocity that depends on the amplitude $A$, the frequency $f$ and the time $t$ is defined as:
\begin{align}
    \omega (t) &= A~2\pi f~\cos(2\pi f~t).
    \label{eq:oscillation_omega}
\end{align}
This definition of the angular velocity implies an angular displacement $\alpha$ of a specific point on the roller surface with the maximum amplitude $A$ which is defined as:
\begin{align}
    \alpha (t) &= A~\sin(2\pi f~t).
    \label{eq:oscillation_alpha}
\end{align}
This angular oscillation can be interpreted in two ways. First, the frequency of the oscillation can help to understand the regime, e.g., above 20 kHz is commonly defined as ultrasonic vibration. Alternatively, the maximum (absolute) circumferential velocity can be related back to an equivalent rotational velocity if the oscillation's maximum speed is taken as the velocity of a constant rotation. That equivalent constant rotational velocity can be easily understood in context of e.g., the results in Section~\ref{subsec:rotational spreading}. For reasons of better interpretation, the amplitude and equivalent rotational velocity are being kept as independent variables and the frequency is chosen as dependent variable. The smallest amplitude is chosen to be approx. half of the median radius of the PSD (with $D50=27\mu m$), which corresponds to 0.08$^{\circ}$ or 7~$\mu m$ of amplitude on the roller surface. By increasing in orders of magnitude, the other examined values are 1$^{\circ}$ (i.e., 87~$\mu m$ amplitude on the roller surface, corresponding to the cutoff diameter of the PSD) and 10$^{\circ}$ (i.e., 873~$\mu m$ amplitude on the roller surface). For the equivalent rotational velocity, values ranging from 10~rpm to 1000~rpm are chosen, which cover approximately the same range as in Section~\ref{subsec:rotational spreading}, while the traverse velocity is constant for all simulations at $25\frac{mm}{s}$, which was identified as best compromise between spreading accuracy and throughput in Section~\ref{subsec:rotational spreading}. Furthermore, a friction coefficient of $\mu = 0.8$ is chosen for all following simulations as it produced the highest packing fractions values. Figure~\ref{fig:rotational study} shows however, that the results for friction coefficients above $\mu = 0.4$ don't meaningfully differ. The full set of parameters is given in Table~\ref{table:oscillation parameters}.

\begin{table}
\centering
\caption{Frequencies for amplitude-'equivalent maximal rotational velocity' combinations of the parameter study}
\label{table:oscillation parameters}
\begin{tabular}{ |p{3.7cm}|r|r|r| } 
 \hline \raggedleft
  Equivalent max rotational velocity in [rpm] &Frequency for 0.08$^{\circ}$ in [Hz] &Frequency for 1$^{\circ}$ in [Hz]           &Frequency for 10$^{\circ}$ in [Hz]\\ 
 \hline
 \raggedleft10    & 119   & 9.55& 0.955 \\ 
 \raggedleft50    & 595   & 47.7 & 4.77\\ 
 \raggedleft100   & 1190      & 95.5 & 9.55\\ 
 \raggedleft250   & 2975      & 239 & 23.9 \\
 \raggedleft500   & 5950      & 477 & 47.7 \\ 
 \raggedleft750   & 8925      & 716 & 71.6 \\ 
 \raggedleft1000  & 11900    & 955 & 95.5 \\
 \hline
\end{tabular}
\end{table}

Figure~\ref{fig:oscillation study} shows the results of the parameter study broken down from two different perspectives. The data points in Figure~\ref{fig:Oscillation_amp} and Figure~\ref{fig:Oscillation_vmax} are the same, but they are plotted on a different legend to allow for deeper understanding of the results. 
Looking at Figure~\ref{fig:Oscillation_amp}, it is evident that for each amplitude, an increase in frequency is generally increasing the packing fraction. Similarly to the pure rotational spreading in Section~\ref{subsec:rotational spreading}, the plateau is followed by a decline for very high frequencies. 
Furthermore, the highest packing fractions are achieved with a medium amplitude around 1$^{\circ}$. This is visible both in Figure~\ref{fig:Oscillation_amp} as well as by the 'hat' shape of the curves in Figure~\ref{fig:Oscillation_vmax} where the middle data point of each curve represents the 1$^{\circ}$-amplitude data point.
From Figure~\ref{fig:Oscillation_amp} it can be concluded that employing a smaller amplitude requires a higher frequency to reach similar results. Shifting the perspective to Figure~\ref{fig:Oscillation_vmax} helps understand this behavior better as each amplitude-frequency combination is mapped to an equivalent maximal rotational velocity. With increasing equivalent maximal rotational velocity, the packing fraction increases, up to 500~rpm. Beyond the peak at 500~rpm, the packing fraction decreases again, similarly to the pure rotational simulations.
Overall, best results are achieved for values between 0.5-5 kHz and amplitudes of 1$^{\circ}$ or below, which corresponds to equivalent maximal rotational velocities around 500~rpm with the employed roller geometry.

\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Roller_oscillation_amp_study_v2.png}
         \caption{Results plotted by oscillation amplitude}
         \label{fig:Oscillation_amp}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Roller_oscillation_vmax_study_v3.png}
         \caption{Results plotted by max circumferential and corresponding rotational velocity}
         \label{fig:Oscillation_vmax}
     \end{subfigure}
     \caption{Mean packing fraction of powder layers spread with angular oscillation for different frequencies and amplitudes}
     \label{fig:oscillation study}
\end{figure}

Qualitative analysis of the particle movement revealed that for very high frequencies and small amplitudes, corresponding to an equivalent velocity above 500~rpm, the inertia of the powder is too high for the roller oscillations to affect the particles. Figure~\ref{fig:high oscillation comparison} shows the exemplary comparison of the highest frequency oscillation (1000~rpm equivalent, 0.08$^{\circ}\approx$~0.1$^{\circ}$ amplitude) and the best layer (500~rpm equivalent, 1$^{\circ}$ amplitude). The arrows indicate the velocity of each particle, with the color being on the same scale as shown in the legend. The length of the arrows for the 1000~rpm case is scaled by a factor of 0.5 compared to the arrows of the 500~rpm case in order to account for the difference in reference velocity of the roller (1000~rpm vs. 500~rpm). In the high frequency case, only particles that are vertically underneath the centerpoint of the roller are affected by the angular movement. This is a typical behavior for a non-rotating/non-oscillating roller where particles in the narrowest part of the gap experience high forces and particles outside that region are largely unaffected. For the best case in Figure~\ref{fig:high oscillation comparison}b, most particles the roller is in contact with are evenly impacted (many similarly sized/colored arrows). This even velocity field indicates strong engagement of the roller with the powder pile. The oscillating nature then allows for a breaking of cohesive bonds between particles and creates a relatively uniform surface. 

\begin{figure}
% \vspace{-12pt}
 \begin{center}
   \includegraphics[width=\textwidth]{Figs/high_oscillation_comparison_v3}
 \end{center}
 \vspace{-16pt}
 \caption{Comparison of powder particle velocities for a) 1000~rpm equivalent with 0.08$^{\circ}$ amplitude and b) 500~rpm equivalent with 1$^{\circ}$ amplitude}
   % \vspace{-12pt}
 \label{fig:high oscillation comparison}
\end{figure}
Comparing the oscillating spreading to the pure rotational spreading, several additional differences are visible. For rotational spreading, the roller surface is completely covered with powder as it adheres to the roller. This is an effect that is also visible in experimental studies performed in our lab. For oscillating spreading, only a small part of the roller surface interacts with the powder and thus has particles adhering to it. Potentially related to that, rotational spreading shows significant ejection of particles from the spreading zone forward onto the powder bed. This creates a kind of dust of particles that are being ejected continuously as the roller moves, especially for high angular velocities. With the oscillating spreading, almost no such dust creation was visible. 
% A comparison of the different scenarios can be observed in supplementary Video 1.



\subsection{Impact of reduced substrate adhesion}
\label{subsec:reduced sadh}

When spreading powder during an LPBF build, it is spread over the previous layer. This means that the substrate is a combination of previously spread powder and melt tracks. The surface properties of powder and melt tracks are quite different and powder particles might adhere differently well. To evaluate the impact of a change in surface properties of the underlying surface (i.e. substrate, powder bed or melt track), the substrate surface energy, as critical parameter for the spreadability, is reduced, which makes the spreading more challenging and allows to assess the robustness of the different spreading strategies. While it is challenging to asses how much the actual surface properties (friction coefficient, contact surface, etc.) between melt track and powder bed differ, we will simply analyze a more extreme case to analyze robustness of the spreading strategies. In this section the substrate surface energy levels are reduced by a factor of 10, meaning that: $\gamma_{substrate, modified} = 0.1\gamma$. For this changed setting, the parameter studies from Section~\ref{subsec:rotational spreading} (for traverse velocity of v = $25 \frac{mm}{s}$) and Section~\ref{subsec:oscillation spreading} (also v = $25 \frac{mm}{s}$) are repeated. 

Figure~\ref{fig:Rotation_low_sadh} shows the results of the equivalent study from Section~\ref{subsec:rotational spreading}. The main insight is that for the roller rotation of $\omega$ = -500 rpm and a roller friction coefficient of 0.4 or larger, the mean packing fraction is comparable to the case with the normal surface adhesion levels of the substrate. E.g., for the case of $\omega$ = -500 rpm and $\mu$ = 0.6, the packing fraction is almost identical (47.0\% for $\gamma_{substrate, modified}$ vs 47.7\% for the default substrate surface adhesion). For friction coefficients $\mu < 0.4$ the powder is not spreadable anymore, a result that is independent of the rotational velocity.
The impact of roller rotation and friction coefficient seems to be significantly more important for a lower substrate adhesion value. For $\omega$ = -250 rpm, the achievable mean packing fraction is comparable to the $\omega$ = -100 rpm case in Section~\ref{subsec:rotational spreading}, however powder is not being spread below $\mu$ = 0.4. For rotational velocities below $\omega$ = -250 rpm, the layer packing fraction is either very low (around 10-15\% for $\omega$ = -100 rpm and $\mu \geq$ 0.6) or no powder is spread at all (all cases below $\omega$ = -100 rpm). In this case, the powder pile is simply being pushed across the substrate without being deposited and no data point is displayed in Figure~\ref{fig:Rotation_low_sadh}.

For the spreading with angular oscillation, the results are similar. The friction coefficient is set to $\mu = 0.8$ for all angular oscillation experiments. For low comparable equivalent maximal rotational velocities, no powder is deposited (e.g., 10 rpm and one 50 rpm scenario which are therefore not plotted). The best spreading results on the other hand are comparable to the best spreading conditions in the unaltered simulations in Section~\ref{subsec:oscillation spreading}. For example, the best result is achieved with $\omega_{equivalent}$ = 500 rpm, amplitude A = 1$^{\circ}$, and frequency f = 4.77e-1 kHz, where the default case had a mean packing fraction of 52.2\% and the scenario with the reduced substrate adhesion achieves 51.5\%.

In summary, while spreading becomes more challenging and in several cases infeasible, the spreading conditions that produce best results on a substrate that has similar cohesive properties as the powder also produce best results on a less cohesive substrate. Even as substrate conditions change significantly, the layer packing fraction stays very consistent which underlines the robustness of these spreading strategies and parameter choices.

\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Roller_v25_rotation_study_low_sadh.png}
         \caption{Spreading with a counter-rotating roller with traverse velocity of v = $25 \frac{mm}{s}$}
         \label{fig:Rotation_low_sadh}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Roller_oscillation_vmax_study_low_sadh_v3.png}
         \caption{Spreading with angular oscillation and a traverse velocity of v = $25 \frac{mm}{s}$ and friction coefficient of $\mu = 0.8$}
         \label{fig:Oscillation_vmax_low_sadh}
     \end{subfigure}
     \caption{Mean packing fraction of powder layers spread over a substrate where the substrate adhesion is reduced by a factor of 10}
     \label{fig:reduced sadh}
\end{figure}




\subsection{Spreading via transverse oscillation and comparison to the other kinematic approaches}

As alternative to the angular oscillation of the roller presented in Section~\ref{subsec:oscillation spreading}, an oscillation can also be applied to the roller normal / transverse to the spreading direction. Therefore, the same roller parameters as in the previous studies are used, i.e., roller diameter $10$~mm, traverse velocity v~=~$25 \frac{mm}{s}$, coefficient of friction for the roller $\mu = 0.8$. Note that this transverse oscillation approach is not limited to rollers. Instead, the roller could e.g. also be replaced by a blade with a circular edge. For the oscillation, the displacement in transverse direction is calculated via $u_y(t) = u_{y0} \sin(2\pi f t)$ with the amplitude $u_{y0}$ and frequency $f$. In the following, the frequencies $f = \{9.55, 47.7, 95.5, 239, 477, 716, 955 \}$~Hz and amplitude $u_{y0} = 0.087$~mm are studied. The amplitude $u_{y0} = 0.087$~mm corresponds to the same displacement as the amplitude $A = 1^{\circ}$ for the angular oscillation based on the same roller diameter, and the frequencies correspond to what it outlined in Table~\ref{table:oscillation parameters}. So, the surface velocity resulting from the oscillation is the same for the angular as well as transverse kinematic, and the maximal surface velocity can be translated into an equivalent angular rotational velocity as well.

Figure~\ref{fig:rotation_oscillation_comp} shows the mean packing fraction for the described frequencies, converted into equivalent angular rotational velocities in rpm. The transverse oscillation is compared to the angular oscillation and pure counter-rotation, both for the base case with similar surface adhesion as well as for the case of reduced substrate surface adhesion by a factor of 10. For the base case, shown in Figure~\ref{fig:Fig13_a}, all three kinematics follow a similar pattern with initially increasing powder layer quality as the (equivalent) angular velocity increases. Transverse oscillation produces the most robust results, spreading powder layers with a consistently high packing fraction across a wide range of frequencies, corresponding to angular velocities of 250~rpm to 1000~rpm.
When the substrate surface adhesion is reduced by a factor of 10 (see Figure~\ref{fig:Fig13_b}), the result is similar. Transverse and angular oscillation produce powder layers with a higher packing fraction than pure angular rotation. Transverse oscillation furthermore has the highest level of consistency across the tested range of oscillation frequencies, a sign of robustness of the kinematic with respect to the spreading parameters as well as the environmental conditions.

Hence, the application of transverse oscillations represents a good alternative to achieve high packing fractions that is applicable to more general spreading tool geometries beyond simple cylindrical shapes.

% \begin{figure}
% % \vspace{-12pt}
%  \begin{center}
%    \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=0.49\textwidth]{Figs/Roller_y-oscillation_v2.png}
%  \end{center}
%  \vspace{-16pt}
%  \caption{Mean packing fraction of powder layers spread with v = $25 \frac{mm}{s}$ and a horizontal oscillation perpendicular to the spreading direction, for different amplitudes and frequencies}
%    % \vspace{-12pt}
%  \label{fig:roller_y_oscillation}
% \end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Fig13_a.png}
         \caption{Comparison with substrate adhesion equal to particle adhesion, traverse velocity of v = $25 \frac{mm}{s}$}
         \label{fig:Fig13_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Fig13_b_v2.png}
         \caption{Comparison with substrate adhesion reduced by a factor of 10, traverse velocity of v = $25 \frac{mm}{s}$}
         \label{fig:Fig13_b}
     \end{subfigure}
     \caption{Mean packing fraction of layers applied by roller spreading with counter-rotation, angular oscillation, and transverse oscillation}
     \label{fig:rotation_oscillation_comp}
\end{figure}


\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Paper2_comparison_low_adh_norm_padh.png}
         \caption{Low adhesion, same substrate adhesion}
         \label{fig:Rotational study 5mms}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Paper2_comparison_low_adh_low_padh.png}
         \caption{Low adhesion, reduced substrate adhesion}
         \label{fig:Rotational study 10mms}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Fig13_a.png}
         \caption{Normal adhesion, same substrate adhesion}
         \label{fig:Rotational study 25mms}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Fig13_b_v2.png}
         \caption{Normal adhesion, reduced substrate adhesion}
         \label{fig:Rotational study 50mms}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Paper2_comparison_high_adh_norm_padh.png}
         \caption{High adhesion, same substrate adhesion}
         \label{fig:Rotational study 25mms}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim = {8mm 0mm 10mm 2mm}, clip, scale=1, keepaspectratio=true, width=\textwidth]{Figs/Paper2_comparison_high_adh_low_padh.png}
         \caption{High adhesion, reduced substrate adhesion}
         \label{fig:Rotational study 50mms}
     \end{subfigure}
     \caption{Caption}
     \label{fig:rotational study supp}
\end{figure}
